Deep Curiosity Loops in Social Environments

Inspired by infants' intrinsic motivation to learn, which values informative sensory channels contingent on their immediate social environment, we developed a deep curiosity loop (DCL) architecture. The DCL is composed of a learner, which attempts to learn a forward model of the agent's state-action transition, and a novel reinforcement-learning (RL) component, namely, an Action-Convolution Deep Q-Network, which uses the learner's prediction error as reward. The environment for our agent is composed of visual social scenes, composed of sitcom video streams, thereby both the learner and the RL are constructed as deep convolutional neural networks. The agent's learner learns to predict the zero-th order of the dynamics of visual scenes, resulting in intrinsic rewards proportional to changes within its social environment. The sources of these socially informative changes within the sitcom are predominantly motions of faces and hands, leading to the unsupervised curiosity-based learning of social interaction features. The face and hand detection is represented by the value function and the social interaction optical-flow is represented by the policy. Our results suggest that face and hand detection are emergent properties of curiosity-based learning embedded in social environments.

==> season_summary.tex <==
\begin{table}
\caption{Summary of dataset, 10 seasons of The Big Bang Theory.}
\centering
\begin{tabular}{cccccc}
\toprule
{} & \multicolumn{3}{c}{Number of Frames} &  {Shots} & {Episodes} \\
\textbf{Season} &             mean &   std &  sum &  &  \\
% \textbf{Season} &                  &       &        &       &         \\
\midrule
\textbf{1     } &            25.71 &  4.51 &  13.96K &   543 &      17 \\
\textbf{2     } &            26.03 &  4.52 &  19.86K &   763 &      23 \\
\textbf{3     } &            26.09 &  4.42 &  19.98K &   766 &      23 \\
\textbf{4     } &            26.12 &  4.42 &  24.48K &   937 &      24 \\
\textbf{5     } &            26.32 &  4.53 &  26.08K &   991 &      24 \\
\textbf{6     } &            26.03 &  4.48 &  21.84K &   839 &      23 \\
\textbf{7     } &            25.66 &  4.40 &  19.76K &   770 &      24 \\
\textbf{8     } &            25.87 &  4.45 &  21.70K &   839 &      24 \\
\cline{1-6}
\textbf{9     } &            25.66 &  4.35 &  19.66K &   766 &      24 \\
\textbf{10    } &            25.68 &  4.45 &  16.46K &   641 &      23 \\
\bottomrule
\textbf{Total } &   \textbf{25.94} &  \textbf{4.46} &  \textbf{203.78K} &   \textbf{7855} & \textbf{229} \\
\\
\end{tabular}


\end{table}


==> temp.tex <==

Both learning objects where trained with Tensorflow \cite{abadi_tensorflow:_2016}, on a single Nvidia Pascal Titan Xp 12GB GDDR5 GPU card. The initialization of the weights was done while staving from introducing outside knowledge, thus where initialized with a random truncated normal distribution, a normal distribution clipped at values 2 standard deviations away from the mean. Its mean was $10^{-4}$ and its standard deviation $10^{-8}$. Every convolution has zero-padding and stride size 1.

\subsection{Learner}

Our Learner $\Phi^L$ is a mapping that aims to learn a forward model of the agent's state-action transition. We chose a convolutional neural network with a single layer with 3 filters of size $7\times 7\times 8$ without pooling and with a ReLU activation, that takes as input an image $I\in S$ ($180\times 320\times 3$) and a one-hot encoding of the actions, $\hat{\textbf{A}} \in \hat{\mathbb{A}}$ (($180\times 320\times 5$)) and outputs a predicted $\hat{I} \in S$, $\Phi^L(I, \hat{\textbf{A}})\mapsto\hat{I}$ ($180\times 320\times 3$). Given the next image $I^\prime \in S$ the learner's cost function, $J^L$ is given by the Mean Squared Error between $\hat{I}$ and $I'$. All together 1176 trained parameters.

\begin{equation}\label{LearnerLoss}
J_L \cbrac{I, \hat{\textbf{A}}, I^\prime} =  \frac{1}{3wh} \sum_{i, j, c} \cbrac{\Phi ^L \cbrac{I, \hat{\textbf{A}}}\sbrac{i, j, c} - I^\prime \sbrac{i, j, c}}^2
\end{equation}

It updates by Stochastic Gradient Descent with momentum \cite{botev_nesterovs_2016}.
Since this is a pure convolutional network, the output (image) is the same size as the input (image), wherein each pixel in the output is affected by $n\times m$ pixels in the input image, centered on it.

\subsection{Intrinsic Rewards Image}

In order to compute the reward we decompose its calculation to two parts. Instead of using the learner's loss directly, we devised a slightly different reward function. First we compute the mean squared difference with respect to each pixel's maximum color value. This results in an image-like value structure with the same dimensions as the input image. Second, we convolve the result with an averaging filter with the same dimensions and zero-padding such that it retains its size. This has the desired affect of averaging with respect to the receptive field of the AC-DQN (see below). This too results in an image-like 2d (no depth/color, or depth 1) structure where every pixel value represents the reward of the state that this pixel represents.

\begin{equation}\label{reward}
\textbf{R} \cbrac{I, \hat{\textbf{A}}, I^\prime} =  \frac{1}{wh} \sum_{i,j}  \cbrac{\max_c \Phi ^L \cbrac{I, \hat{\textbf{A}}}\sbrac{i, j, c} - \max_c I^\prime \sbrac{i, j, c}}^2
\end{equation}

% Although this deviates from the Curiosity loop, it is amenable to our implementation. To generate the correct rewards, instead of acting on the next frame before the Learner predicts we act on it afterwards while also acting on the prediction itself. Only then we compute the rewards for that time step. Despite looking like a divergence from the Curiosity Loop, this is only a detour. The reason is that for every kind of action this mimics its correct influence on the prediction. Say we want to predict the next frame given that the agent moved one way by $k$ steps, than the Learner should have generated the same prediction but with the entire image shifting the opposite direction by the same $k$. Put another way, the agent looking up by 5 pixels is equivalent to a static Learner's entire prediction shifting down by 5 pixels.

\subsection{Action-Convolution Deep-Q Network}

With the intention of parallelizing the Deep Curiosity Loop we devised a new algorithm called Action-Convolution Deep-Q Network (AC-DQN). 
It is a variant of Deep Q-Network (DQN) and Double Deep Q-Network (DDQN). These networks are essentially $Q$ function approximators that employ the Deep CNN structure and learn through gradient descent (ADAM \cite{kingma_adam:_2014}) to minimize the TD-error. As with both algorithms, we make use of Experience Replay (prioritize \cite{schaul_prioritized_2015}). Between layers we use instance normalization \cite{ulyanov_instance_2016} which does not require turning off after learning.

AC-DQN is a deep CNN architecture $\Phi^Q$ with an image as its input and a matrix with the same height $h$ and width $w$ as the reward. The network's last layer is of dimensions $h \times w \times \vert A \vert$, where $A$ is the action space.
We are using DDQN, hence the target $\textbf{T}$ is the matrix-addition of the reward matrix (``image'') and the discounted approximation of the output of $\Phi^Q$ on the next frame, and the TD-error is denoted as $\delta$.

\begin{equation}\label{TD}
\textbf{T} = \textbf{R} + \gamma \cdot \max_{\hat{\textbf{A}} \in \hat{\mathbb{A}}} \Phi^Q\cbrac{I^\prime, \hat{\textbf{A}}} \quad
\delta = \vert \Phi^Q \cbrac{I, \hat{\textbf{A}}} - T \vert
\end{equation}

The final AC-DQN version uses a DCNN with 10 convolutional layers. Each hidden layer has a filter depth of 30 with ReLU activations whereas the output layer has depth 5 to match the number of actions. This layer has a linear activation function. 
Each layer's filter dimensions is $5\times 5$ except the first for which is $9\times 9$. 
Effectively, the AC-DQN has a receptive field of $45\times 45$ with respect to the input layer. \add{All in all the network trained with 191040 parameters.}

The novelty of our proposed AC-DQN architecture is in its output layer.
In traditional in DQN variants, given input $s$, the output of the network is a vector where the entry for each action $a$ represents the prediction of $Q\cbrac{s, a}$. 
However, in order to parallelize the Deep Curiosity Loop our AC-DQN's output is a matrix with the hight and width of the input image $I$ and with depth the size of the action space (here $\vert A \vert = 5$).
In essence, we compute the Q-value for {\em each pixel} (environment) in the input image. Consequently, AC-DQN's loss function is actually the mean of the TD-error over all pixels.
